Near-Optimal Massively Parallel Graph Connectivity

Identifying the connected components of a graph, apart from being a fundamental problem with countless applications, is a key primitive for many other algorithms. In this paper, we consider this problem in parallel settings. Particularly, we focus on the Massively Parallel Computations (MPC) model, which is the standard theoretical model for modern parallel frameworks such as MapReduce, Hadoop, or Spark. We consider the truly sublinear regime of MPC for graph problems where the space per machine is $n^\delta$ for some desirably small constant $\delta \in (0, 1)$. We present an algorithm that for graphs with diameter $D$ in the wide range $[\log^{\epsilon} n, n]$, takes $O(\log D)$ rounds to identify the connected components and takes $O(\log \log n)$ rounds for all other graphs. The algorithm is randomized, succeeds with high probability, does not require prior knowledge of $D$, and uses an optimal total space of $O(m)$. We complement this by showing a conditional lower-bound based on the widely believed TwoCycle conjecture that $\Omega(\log D)$ rounds are indeed necessary in this setting. Studying parallel connectivity algorithms received a resurgence of interest after the pioneering work of Andoni et al. [FOCS 2018] who presented an algorithm with $O(\log D \cdot \log \log n)$ round-complexity. Our algorithm improves this result for the whole range of values of $D$ and almost settles the problem due to the conditional lower-bound. Additionally, we show that with minimal adjustments, our algorithm can also be implemented in a variant of the (CRCW) PRAM in asymptotically the same number of rounds.

==> algorithmictools.tex <==
\section{Basic Algorithmic Tools for \MPC{}}
In this section we describe a set of basic algorithmic primitives for graph problems in the \MPC{} model.

\input{load-balancing-brief}
\input{gathering.tex}

==> applications.tex <==
\section{Applications}

\subsection{Spanning Forest}\label{sec:spanning-forest}

In this section we show that the connectivity algorithm from
Section~\ref{sec:algorithm} can be extended to compute a spanning forest using
asymptotically the same number of rounds. We describe an algorithm
that based on the algorithm presented by Andoni et al, which we first
review.

\newpara{The Andoni et al. Algorithm}
The Andoni et al. spanning forest algorithm is based on computing a
local shortest path tree rooted at each vertex while path-doubling. A
\emph{local shortest path tree (LSPT)} rooted at a vertex $u$ is a
tree containing the shortest path distances (hop-distance) between $u$
and the vertices in the tree. The LSPTs produced by the algorithm have
additional structure that is helpful: roughly, the LSPT of a vertex
that has performed $i$ rounds of adding-edges consists of all vertices
that are $2^i$ hops away from the vertex. The LSPT of a vertex $u$ is
represented as follows: for each neighbor $v \in N(u)$, we store the
parent of $v$ in the LSPT and the shortest path distance between $u$
and $v$ (the hop distance). An LSPT can be maintained by observing
that when we add edges, we can afford to compute the minimum distance
to a new neighbor $w$, by computing $\min_{v \in N(u)} d(u, v) + d(v,
w)$. The parent is updated by taking the parent of $w$ in the LSPT of
the neighbor $v$ that minimizes the above expression.  Viewed another
way, the adding edges step in the algorithm repeatedly computes the
min-plus product (matrix squaring over the min-plus semiring) over a
subset of vertices until the budget constraint of the vertices is met.

The next part of their algorithm concerns leader selection. As in the
connectivity algorithm, once each vertex hits its budget, a subset
of leaders is selected at random, with probability inversely
proportional to the current budget. However, instead of picking an
arbitrary leader for each non-leader vertex, leaders are chosen by
using the LSPTs in a way that ensures that a spanning tree can be
incrementally built. Each non-leader vertex, $u$, first computes the
distance to the closest leader vertex in its LSPT. Then, it either
chooses some leader vertex if a leader is one-hop away in the
original graph, or chooses a neighboring node that is one hop closer
to a leader vertex. The edge between $u$ and the chosen node is
included as part of the spanning forest. The algorithm also maintains
a mapping from the current set of edges to the original edge-set,
which can be used to obtain a spanning forest in the original graph.
The last step is to use path-doubling to compute the leaders chosen by
each vertex, which costs $O(\log D)$ rounds (this is not a bottleneck
as each adding-edges phase costs $O(\log D)$ rounds in their
algorithm). The main property used to obtain a spanning forest is that
the subgraph induced by all chosen edges for nodes that relabel to
some leader $l$ forms a connected subgraph.

\newpara{Modifications}
Our spanning forest algorithm is similar to the Andoni et al.
algorithm, but requires modifications due to the fact that we
interleave adding-edges and relabeling. Another problem is that we
cannot afford to spend $O(\log D)$ rounds after relabeling in order to
find the leader selected by each non-leader vertex. In what follows we
distinguish between \emph{real edges} which are edges that correspond
to some edge in the original graph and \emph{virtual edges} which are
edges that we add in order to boost the degrees through adding-edges
steps. We use $N_{R}(u)$ to denote the real neighbors of $u$ at the
current step. We say that a vertex $u$ is \emph{affected} if there
exists $v \in N(u)$ that has participated in a relabeling step, and
\emph{unaffected} otherwise.

Instead of selecting representatives in the relabeling steps by using
path-doubling (and spending $O(\log D)$ rounds to compute the leader
or high-degree vertex the relabeled vertex contracts to), we argue
that each relabeled vertex can locally select a real edge incident to
it so that the subgraph induced by the chosen (real) edges in this
step relabeling to some vertex, $l$, form a connected subtree rooted
at $l$. Given this property, arguing that we produce a spanning forest
follows by induction.

We also distinguish between affected and unaffected vertices because
affected vertices may not be able to consistently contract themselves
into their leader, as some of their neighbors may have relabeled
themselves. The relabeled neighbors can interfere with the desired
consistency property along real edges for relabeling vertices. We
observe that affected vertices can be handled by using structural
properties of the shortest path trees built by the algorithm that
allow us to handle affected vertices by just waiting one round and
allowing the vertex to perform an inter-level relabeling.

We start with some basic facts about the LSPTs produced by Algorithm
6 (Large Local Shortest Path Trees) from Andoni et al.

\begin{fact}
  $\forall v \in V \setminus V_{T_{u}}, w \in LSPT(u)$ we have
  $\dist(w, u) \leq \dist(v, u)$. (Lemma C.7 in Andoni et al.)
\end{fact}

\begin{lemma}
If $v, w \in LSPT(u)$, and $v$ is along the shortest path between $u$
and $w$, then $w \in LSPT(v)$.
\end{lemma}
\begin{proof}
  The LSPT produced by Algorithm 6 in Andoni et al. is either an LCPST
  or the vertex's original neighbors plus the neighbors of one of its
  large-degree neighbors (this case can be viewed as an LCSPT where a
  subset of the neighbors violate the radius of the LCSPT by exactly
  one). Sort the neighbors chosen for a large-degree vertex (line 19
  in Algorithm 6) by their id in order to ensure consistency.
\end{proof}

\begin{lemma}\label{lem:consistent}
  Let $L \subseteq V$ be a set of representatives. Consider $u \in V$
  undergoing relabeling to $l(u) = \arg \min_{l \in L} \dist(u, l)$,
  breaking ties by picking the vertex with lowest id.
  Let $v \in N_{R}(u)$ s.t. $\dist(v, l) = \dist(u, l) - 1$ (such a
  vertex exists by induction). For the sake of the current relabeling
  step, we say $u$ chooses the $(u,v)$ edge.
  The set of chosen edges for vertices that select some $l \in L$ form
  a connected tree rooted at $l$.
\end{lemma}
\begin{proof}
The proof is by contradiction. If the set of vertices that relabel to
some $l \in L$ do not form a connected tree, then there exists a vertex
$u$ that relabels to $l$ where there is no continuous path between $u$
and $l$ on the chosen edges. Therefore, $l$ is not a real neighbor of
$u$, so there must be some $v$ along the shortest path from $u$ to $l$
s.t. $v$ does not relabel to $l$. If $l(v) \neq l(u)$, then there are
two possibilities: either $l(v) \notin N(u)$ or $l(u) \notin l(v)$. We
show that neither case can occur and then show that this implies $l(u)
= l(v)$, contradicting the fact that the path from $u$ to $l$ is
broken by $v$.
\end{proof}

\subsection{Rooted Spanning Forest}
The trees generated at each level are rooted at a \emph{selected
  vertex} (either a leader or high-degree vertex). For each tree, we
spend $O(\log D)$ time to compute the size of the subtree rooted at
each node. These operations can be pipelined which lets us compute all
subtree sizes for all trees in the same complexity as the unrooted
spanning tree algorithm. If a tree has size larger than $n^{\epsilon}$
we split it into pieces of size $n^{\epsilon}$ each based on the
augmented sizes.

The re-rooting algorithm works exactly as in Andoni et al., the only
difference is the implementation.  Re-rooting small trees can clearly
be done in one round as they fit on one machine. A large tree can be
re-rooted in $O(1)$ rounds by observing that we can build a tree with
depth $O(1/\epsilon)$ that provides shortcuts to all ancestors of a
block in the tree. I'm eliding basically all of the details on how to
compute this shortcut structure but it seems like something like this
can go through and let us perform the path-computation in $O(1)$
rounds after paying $O(\log D)$ pre-processing time.

\subsection{Tree Operations}
TODO: describe the tree-primitives available in the model. I think
these are pretty much imported from Andoni et al.

\subsection{Tarjan-Vishkin's Biconnectivity Algorithm}
TODO

\subsection{More notes on Andoni et al.}

They distinguish between LSPT (local shortest path tree) and LCPSTs
(local complete shortest path tree). A $LSPT(u)$ is represented as a
tuple $(V_{T}, \texttt{par}_{T})$, which are the vertices in the tree
and tuples mapping vertices to their parents in the tree. LSPTs have
the property that $\forall v \in V_{T}, \texttt{depth}_{T}(v) =
\dist(u, v)$ (the tree distance is the shortest path distance in $G$).
LCPSTs are LSPTs that have the additional property that $V_{T} =
B_{G}(u, s)$ for some radius $s \geq 1$.

The basic algorithm is \emph{TreeExpansion} (Algorithm 4). This takes
in a LCSPT and spits out a LCSPT with twice the radius (initially
$N(u)$ is an LCSPT).

The \emph{MultiRadiusLCSPT} algorithm (Algorithm 5) is a wrapper around
TreeExpansion that ensures vertices don't violate the per-vertex
budget. The algorithm generates one LCPST per vertex, per round. A
vertex keeps doubling via TreeExpansion until either (1) it notices
that a neighbor has hit its budget, or (2) it has a neighbor that's
hit its budget. Once either of these conditions are met is sets its
LCPST for this round to null. The algorithm runs for $r = O(\min(\log
D, m / n))$ rounds. The output is $r$, the number of rounds, $r$ trees
for each vertex representing the LCPST on that round, and the depths
of vertices in each of these trees.

\newpara{The glue:} Finally the \emph{Large Local Shortest Path Trees}
algorithm (Algorithm 6) combines the LCPSTs generated in
MultiRadiusLCSPT to generate LSPTs. The output is an LSPT per vertex
and the depth per tree. Some variables: $\tilde{T}(v)$ is the output
LSPT.  $\tilde{T}_{i}(v)$ is the LCPST for $v$ on step $i$. $s_{i}(v)$
is the radius  of LCSTPT on step $i$, with dep defined similarly for
the depth on round $i$.

The algorithm first generates trees with different radii using
MultiRadiusLCSPT. It then separately handles trees with $T_{r}(v) =
\texttt{null}$ and those with $T_{r}(v) \neq \texttt{null}$. If
this last round tree is non-null, we have a spanning-tree for the
component $v$ belongs to, so we set the output LSPT to this tree and
are done. Otherwise, at some round $r' < r$, we stopped generating
the LCPST for $v$ as the size of its ball grew larger than $d$.



==> biconnectivity.tex <==

\subsection{Biconnectivity}

\newcommand{\codevar}[1]{\mathit{#1}}
\begin{algorithm}[!t]
\caption{Biconnectivity} \label{alg:biconnectivity}
\small
\begin{algorithmic}[1]
\Procedure{Biconnectivity}{$G(V, E)$}
\State $\codevar{F}$ = \textproc{RootedSpanningForest}($G$)
\State $\codevar{PN}$ = \textproc{PreorderNumber}($F$)
\State For each $v \in V$, compute $\codevar{Low}(v)$ and $\codevar{High}(v)$ and $\codevar{Size}(v)$
\State $\codevar{critical}$ = $e = (u, p(u)) \in F$ s.t. $p(u)$ is an articulation point
\State $\codevar{Labels}$ = \textproc{CC}($G(V, E \setminus \codevar{critical})$)
\State \algorithmicreturn{} $(\codevar{Labels}, F)$ \Comment{sufficient to answer biconnectivity queries}
\EndProcedure
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:biconnectivity} shows the Tarjan-Vishkin
biconnectivity algorithm~\cite{tarjan1985efficient}.  We describe our
implementation of this algorithm in more detail in
Section~\ref{sec:algs}.  We first compute a spanning forest of $G$
using the work-efficient connectivity algorithm, where the trees in
the forest can be rooted arbitrarily (Line 2). Next, we compute a
preorder numbering, $\codevar{PN}$, with respect to the roots (Line
3). We then compute for each $v \in V$ $\codevar{Low}(v)$ and
$\codevar{High}(v)$, which are the minimum and maximum preorder
numbers respectively of all non-tree $(u, w)$ edges where $u$ is a
vertex in $v$'s subtree. We also compute $\codevar{Size}(v)$, the size
of each vertex's subtree. Note that we can determine whether the
parent of a vertex $u$ is an articulation point by checking
$\codevar{PN}(p(u)) \leq \codevar{Low}(u)$ and $\codevar{High}(u) <
\codevar{PN}(p(u)) + \codevar{size}(p(u))$. We refer to this set of
tree edges $(u,p(u))$, where $p(u)$ is an articulation point, as
\emph{critical edges}. The last step of the algorithm is to solve
connectivity on the graph with all critical edges removed. Now, the
biconnectivity label of an edge $(u,v)$ is the connectivity label of
the vertex that is further from the root of the tree. The query data
structure can thus report biconnectivity labels of edges in $O(1)$
time using $2n$ space.

We need to argue that the second connectivity call also works on a
graph with diameter $\mathsf{poly}(D)$. In fact, the diameter of the
graph with all critical edges removed can be at most $D$ by a simple
argument. Let $G' = G(V, E \setminus \codevar{critical})$. AFSOC that
some component in $G'$ has diameter larger than $D$, i.e. there is a
shortest path in $G'$ between two vertices $u, v$ of length longer
than $D$. Because this component is a biconnected component, we know
that the critical edges cannot participate in a shorter path, as there
is no way to exit the component via a critical edge and reconnect to
some other vertex in the component. Therefore, this shortest path with
length larger than $D$ is also present in $G$, which is a
contradiction. As a result, the second connectivity call also runs on
a graph with $O(m)$ edges and diameter at most $D$.


